Interplay between Social Influence and Network Centrality: A Comparative Study on Shapley Centrality and Single-Node-Influence Centrality

We study network centrality based on dynamic influence propagation models in social networks. To illustrate our integrated mathematical-algorithmic approach for understanding the fundamental interplay between dynamic influence processes and static network structures, we focus on two basic centrality measures: (a) Single Node Influence (SNI) centrality, which measures each node's significance by its influence spread; and (b) Shapley Centrality, which uses the Shapley value of the influence spread function --- formulated based on a fundamental cooperative-game-theoretical concept --- to measure the significance of nodes. We present a comprehensive comparative study of these two centrality measures. Mathematically, we present axiomatic characterizations, which precisely capture the essence of these two centrality measures and their fundamental differences. Algorithmically, we provide scalable algorithms for approximating them for a large family of social-influence instances. Empirically, we demonstrate their similarity and differences in a number of real-world social networks, as well as the efficiency of our scalable algorithms. Our results shed light on their applicability: SNI centrality is suitable for assessing individual influence in isolation while Shapley centrality assesses individuals' performance in group influence settings.

==> discussion.tex <==


\section{Discussions and Things to Do}

%Wiki quote:
%% In graph theory and network analysis, indicators of centrality identify the most important vertices within a graph. Applications include identifying the most influential person(s) in a social network, key infrastructure nodes in the Internet or urban networks, and super-spreaders of disease. Centrality concepts were first developed in social network analysis, and many of the terms used to measure centrality reflect their sociological origin.[1] They should not be confused with node influence metrics, which seek to quantify the influence of every node in the network.

%% Centrality indices are answers to the question ``What characterizes an important vertex?'' The answer is given in terms of a real-valued function on the vertices of a graph, where the values produced are expected to provide a ranking which identifies the most important nodes.[2][3]

%% The word ``importance'' has a wide number of meanings, leading to
%% many different definitions of centrality. Two categorization
%% schemes have been proposed. ``Importance'' can be conceived in
%% relation to a type of flow or transfer across the network. This
%% allows centralities to be classified by the type of flow they
%% consider important.[3] ``Importance'' can alternately be conceived
%% as involvement in the cohesiveness of the network.

\wei{
I think we need to tight down our page usage, since currently it is likely to be significantly over the page limit.
The following is my rought estimate of the page budget for each section, based on my past experience, and some comments
on the main points to focus on each section.

\begin{itemize}
	\item 
	Abstract, intro, related work, 2 pages, we can talk about general impact of Shapley value, but perhaps need to focus more on network influence.
	Our main contributions are: (a) provide a near linear-time algorithm to compute Shapley value for a large class of influence model, despite that
	Shapley value definition depends on the numeration of all permutations, and influence computation are typically \#P-hard.
	(b) provide an axiomatization talored for networked influence. The axioms are on the general probabilistic influence model, with more degree of freedom than
	characteristic functions, and also has constraint on normalization, but yet still we are able to derive the uniqueness of the solution using Shapley value.
	(c) conceptual discussion on the use of Shapley value.
	\item
	Preliminaries, try to cover it within 1 page, or even shorter.
	\item Efficient algorithm {\ASVRR}, this can be covered in 1 page, but since it is the major algorithmic contribution, 1 page may seem short for
	reviewers. 1 - 1.5 pages. All the proof will be moved to appendix. I can add some explanations on the key ideas leading to the design of the algorithm,
	which is not very hard.
	\item
	Axiomatization, at most 2 pages, giving the axioms and the results. 
	\item
	Discussion on shapley centrality, including the counter-intuitive symmetric IC model result. I think this part needs to be limited, avoid discussing too much
	on the general impact. Since many general conceptual discussion without technical backup may not convince the reviewers. 
	\item Experiments, at least 3 pages. I checked my past kdd papers, and they have at least 3 pages of experiments, and I think for this paper we need that
	space too.
	\item reference, we don't have space left, so we need to make some space, and also try to restrict reference to 0.5 page or a bit more.
\end{itemize}
	
	
	}




\begin{itemize}
\item Need to study if the exact computation of the Shapley value is NP-hard
	for IC and other models.

\item Characterization of influence models with scalable 
  Shapley approximation.

\item Characterization of influence models with polynomial-time
  Shapley approximation.

\item Characterization of influence models with intractable
  Shapley approximation.


	

	
\item We need a problem to show that using relative error bound relative to 
	$\sigma^*_1$ is useful. Probably a direct application is to find the 
	top-$k$ nodes with the largest Shapley values, or find nodes with
	Shapley values larger than a threshold $\Delta$.
	
\item Is it possible to adaptively control the number of RR sets sampled to select
	nodes with large Shapley values?
	
\item What is the best way to justify the use of Shapley value for influence functions?
In particular, if we use axiomatic approach of Shapley values as justification, we
	should think of the practical meaning of additions of two influence functions.
Influence function multiplied by a scalar makes sense to me.
Perhaps need to check the derivation of the uniqueness of the Shapley value.

\item Can the result be extended to weighted case (nodes have weight)?

\item Shapley extension for Hubs-Authorities?

\item Learning Centrality from influence data: Stability of Shapley values

\item Network inference from centrality

\item Learning social influence model from ???

\end{itemize}


==> spreadaxiom.tex <==
\section{Influence-Spread-based\\ Axiomatic Characterization} \label{app:spreadaxiom}

The axiomatic characterization presented in Section \ref{sec:Axioms} 
 has the remarbable property that its unique solution is fully determined by 
 the influence-spread profile, whose dimensionality is much lower than that of
  the probability-distribution profile of the influence model.
To gain more understanding of the axiomatic characterization, 
  in this section, we study the following question:
Do we need to keep all axioms of Section \ref{sec:Axioms} for the 
  representation theorem, 
   if we make this property explicit by introducing it as an axiom:

\begin{axiom}[Spread Determination] \label{axiom:spread}
For two influence instances $\calI_1 = (V, E, P_{\calI_1})$ 
  and $\calI_2 = (V, E, P_{\calI_2})$ on the same graph $G=(V,E)$, 
  if $\sigma_{\calI_1} = \sigma_{\calI_2}$, then $\psi(\calI_1) = \psi(\calI_2)$.
\end{axiom}

In this section, we prove that the
   Axiom Isolated Node  (Axiom~\ref{axiom:isolated})
   can be replaced by the Axiom Spread Determination.
Equivalently, if we replace Axiom Spread Determination (which reduce the dimenionality of the axiomatic characterization) by the simple
 Axiom Isolated Node, then 
 we extend the influence-profile based axiomatic characterization to
 the influence-distribution based axiomatic characterization.

\subsubsection*{{\sc Influence-Profile Based Axiom Set}}

Let $\cA_\sigma$ denote the set of Axioms
  after replacing  Axiom Isolated Node in $\cA$ with Axiom Spread Determination.
In other words, $\cA_\sigma$ consists of Axioms 1-2 and 4-7.
It follows from Theore, \ref{thm:ShapleyCen}:
\begin{corollary}[Soundness]
The Shapley centrality also Axiom set $\cA_\sigma$.
\end{corollary}
%It is trivial to see that the Shapley centrality also 	satisfies Axiom~\ref{axiom:spread}, and thus the main change of the proof is the
In this section, we prove that the Shapley centrality remains
  the unique solution to $\cA_\sigma$.
Because the centrality measure is fully determined 
  by the influence spread, this uniqueness proof is in fact much
  simpler than the one for the axiom set $\cA$.

\subsubsection*{{\sc Activated vs Influenced}}

Our analysis below in fact shed light on another interesting question about
  social-influence:
Shall we measure the influence-spread by the expected size of the set it 
 {\em  activated} in the influence process, or shall we 
  measure the influence-spread by the expected size of the set it 
  {\em actually influenced} during the influence process?
The former is given by $\sigma(S) = \E[|\bI(S)|]$.
The latter is given by $\sigma'(S) = \E[|\bI(S)|-|S|] = \E[|\bI(S)|]-|S|$.

Mathematically, how is the ranking given by the Shapley value of 
  the social-influence game with $\sigma$ as the characteristic function
  related to the Shapley value of 
  the social-influence game with $\sigma'$ as the characteristic function?
Before studying the characterization of Axiom set $\cA_\sigma$, 
  we first give the following connection about these two Shapley values.

\begin{lemma}[Activated vs Influenced]\label{lem:AI}
For any influence instance $\calI$ and
	any subset $S \subseteq V$,
  let $\sigma'_\calI(S) = \sigma_\calI(S) - |S|$.
Then:
\[\phi_v^{Shapley}(\sigma'_\calI) = \phi^{Shapley}_v(\sigma_\calI) -1, \quad 
\forall v\in V.\]
%Let $\psi'$ be the centrality measure derived from the   Shapley value of $\sigma'_\calI$,	that is $\psi'(\calI) = .Then $\psi'$ is a solution to axiom set $\cA'$.
\end{lemma}
\begin{proof}
%First, we have
\begin{align*}
& \phi^{Shapley}_v(\sigma'_\calI) \\
& =  \E_{\bpi}[\sigma'_\calI(S_{\bpi,u} \cup \{u\}) - \sigma'_\calI(S_{\bpi,u})] \\
	 & =  \E_{\bpi}[\sigma_\calI(S_{\bpi,u} \cup \{u\}) - |S_{\bpi,u} \cup \{u\}| - (\sigma_\calI(S_{\bpi,u}) - |S_{\bpi,u}|)] \\
	 & =  \E_{\bpi}[\sigma_\calI(S_{\bpi,u} \cup \{u\}) - \sigma_\calI(S_{\bpi,u})] - 1\\
	 & =  \phi^{Shapley}_v(\sigma_\calI) - 1. % = \psi^{Shapley}_v(\calI) - 1,
\end{align*}
%where $\psi^{Shapley}$ is the Shapley centrality.
%Then since  $\psi^{Shapley}$ satisfies
%	axiom set $\cA_\sigma$, by Lemma~\ref{lem:oneone}, we know that $\psi'=\psi^{Shapley} - 1$ satisfies axiom set $\cA'$.
\end{proof}
Lemma \ref{lem:AI} shows that from the Shapley value perspective, 
  using the number of activated nodes  and the number of influenced nodes
  for measuring influence spread are fundamentally equivalent.
%influence-spread by the   is equivalent to  influence-spread profiles by  is equivalent

\subsubsection*{{\sc An  Equivalent Axiom Set}}

%% The following is the old analysis relying on the Spread Axiom, and making connection to function $\sigma'_\calI(S) = \sigma_\calI(S) - |S|$.
To facilitate the uniqueness proof, 
  we study a similar set of axioms $\cA_{\sigma'}$, such that
  while the unique solution to $\cA_\sigma$ is 
  the Shapley value $\phi^{Shapley}(\sigma_\calI)$, 
  the unique solution to $\cA_{\sigma'}$ is 
  the Shapley value $\phi^{Shapley}(\sigma'_\calI)$
  of $\sigma'_\calI(S) = \sigma_\calI(S) - |S|$.

As discussed above, function $\sigma'_\calI(S)$ 
  reflects in some sense the net payoff for selecting seed set $S$,
  since the additional influence $\sigma_\calI(S) - |S|$ 
  are usually considered as the actual gain.
Therefore, besides serving as a vehicle to prove the uniqueness of the axiom set
	$\cA_\sigma$, understanding axiom 
  set $\cA_{\sigma'}$ and its relationship to $\cA_\sigma$ has its independent
  benefit.

Axiom set $\cA_{\sigma'}$ replaces Axiom~\ref{axiom:normalization} and~\ref{axiom:critical} 
	in $\cA_\sigma$ with
	the following Axiom~2' and Axiom~6', while keeping the rest four axioms 
	in $\cA_\sigma$ unchanged.

\vspace{2mm}
\noindent
{\bf Axiom 2'.} \ \
{\em 
	For every influence instance $\calI = (V,E,\calD)$, $\sum_{v\in V} \psi_{v}(\calI)  = 0$.
}

\vspace{2mm}
\noindent
{\bf Axiom 6'.} \ \
{\em 
In any critical set  instance
$\calI_{R,v}$, \remove{ = (R\cup\{v\}, \{(u,v): u\in R\}, P_{\calI_{R, v}})},
%If an influence instance $\calI = (V,E, \calD)$ has a critical set $R$ and $V \setminus R = \{v\}$, then 
it should be the case that $\psi_v(\calI_{R,v}) = -\frac{1}{|R|+1}$. 
}
\vspace{2mm}

Motivated by Lemma \ref{lem:AI}, we define the following:
%We first build the one-to-one correspondence between the centrality measures in the two	axiom sets.
Let $\psi$ be a centrality measure. 
We define $(\psi-1)$ to be the centrality measure 
	such that for every influence instance
	$\calI$ and for every node $v$, $(\psi-1)_v(\calI) = \psi_v(\calI) - 1$.
Similarly, we define $(\psi+1)$.
Clearly, 
$((\psi+1)-1)$, $((\psi-1)+1)$, and $\psi$ are the same centrality measure,
  for any centrality measure $\psi$.


\begin{lemma}[One-to-One] \label{lem:oneone}
A centrality measure  $\psi$ satisfies 
  axiom set $\cA_\sigma$ if and only if $(\psi-1)$ is a centrality
	measure satisfying axiom set $\cA_{\sigma'}$.
%Conversely, if $\psi'$ is a centrality measure satisfying axiom set $\cA'$, then	$\psi'+1$ is a centrality measure satisfying axiom set $\cA_\sigma$.
\end{lemma}
\begin{proof}
Suppose that $\psi$ is a centrality measure satisfying axiom set $\cA_\sigma$.
Axioms~\ref{axiom:anonymity}, \ref{axiom:spread}, \ref{axiom:sink}, and \ref{axiom:bayesian}
	do no change between $\cA_\sigma$ and $\cA_{\sigma'}$, 
and $(\psi-1)$ is only a constant change from $\psi$,
	so $(\psi-1)$ also satisfies these axioms.
Axioms~\ref{axiom:normalization} and~\ref{axiom:critical} are changed to
	Axioms 2' and 6' respectively, 
  which can be achieved exactly by reducing the centrality
	of each node by $1$, and thus $(\psi-1)$ satisfies Axioms 2' and 6'.
Symmetrically, on-if statement can be proved.
\end{proof}
Lemma~\ref{lem:oneone} above establishes the one-to-one correspondence between 
	solutions to axiom set $\cA$ and solutions to axiom set 
$\cA_{\sigma'}$, which means if
	we can prove that the solution to $\cA_{\sigma'}$ is unique, 
  we also proves that the solution to $\cA_\sigma$ is unique.
But before that, we give the following connection with Shapley value.
\begin{lemma}[Soundness]
%Let $\sigma'_\calI(S) = \sigma_\calI(S) - |S|$, for any influence instance $\calI$ and 	any subset $S \subseteq V$.
Let $\psi'$ be the centrality measure 
  derived from the Shapley value of $\sigma'_\calI$,
	that is, $\psi'(\calI) = \phi^{Shapley}(\sigma'_\calI)$.
Then $\psi'$ satisfies $\cA_{\sigma'}$.
\end{lemma}
\begin{proof}
%% First, we have
%% \begin{align*}
%% & \psi'_v(\calI) = \phi^{Shapley}_v(\sigma'_\calI) \\
%% & =  \E_{\bpi}[\sigma'_\calI(S_{\bpi,u} \cup \{u\}) - \sigma'_\calI(S_{\bpi,u})] \\
%% 	 & =  \E_{\bpi}[\sigma_\calI(S_{\bpi,u} \cup \{u\}) - |S_{\bpi,u} \cup \{u\}| - (\sigma_\calI(S_{\bpi,u}) - |S_{\bpi,u}|)] \\
%% 	 & =  \E_{\bpi}[\sigma_\calI(S_{\bpi,u} \cup \{u\}) - \sigma_\calI(S_{\bpi,u})] - 1\\
%% 	 & =  \phi^{Shapley}_v(\sigma_\calI) - 1 = \psi^{Shapley}_v(\calI) - 1,
%% \end{align*}
By Lemma \ref{lem:AI}, $\psi' = (\psi^{Shapley}-1)$,
 where $\psi^{Shapley}$ is the Shapley centrality.
Since  $\psi^{Shapley}$ satisfies
	axiom set $\cA_\sigma$, by Lemma~\ref{lem:oneone}, 
we conclude  %that $\psi'=\psi^{Shapley} - 1$ 
 $\psi'$   satisfies axiom set $\cA_{\sigma'}$.
\end{proof}
 %% the following is the old proof using the Spread axiom, and is based on the mapping from spread function to vector.
\begin{lemma}[Uniqueness] \label{lem:unique2}
	The centrality measure satisfying axiom set $\cA_{\sigma'}$ is unique.
\end{lemma}
\begin{proof}
Fix a vertex set $V$. % graph $G=(V,E)$.
Let $\psi'$ be a centrality measure that satisfies axiom set $\cA_{\sigma'}$.
For any $R \subset V$ and $R\ne \emptyset$,
let $\calI_R$ be an influence instance $\calI_R = (V,E, \calD_R)$
in which $R$ is the critical set and $V$ is the target set, 
	i.e., $\calI_R$ is a shorthand for $\calI_{R,V}$.
By the Anonymity Axiom (Axiom~\ref{axiom:anonymity}), all nodes in $R$ have the same
centrality measure, say $a_R$,
   and all nodes outside $R$ have the same
  centrality measure, say $b_R$.
By Axiom 2', we have
$a_R \cdot |R| + b_R \cdot (|V|-|R|) = 0$.	
Consider any node $v\not\in R$.
By Lemma~\ref{lem:isosink}, $v$ is a sink node.
Then, we can apply Axiom  Sink Node (Axiom~\ref{axiom:sink}) to iteratively
  remove all but the last node $v\not\in R$, 
  such that the central measure of $v$ does not change after the removal.
It follows from the definitions of projection and critical set instance
%Definitions~\ref{def:projection} and~\ref{def:critical} 
that  $R$ is still the critical set for the resulting instance.
Thus, by Axiom 6', the centrality measure of $v$ is $-1/(|R|+1)$, i.e., 
   $b_R = -1/(|R|+1)$.
Therefore, $a_R = (|V|-|R|)/(|R|(|R|+1))$ 
  is also uniquely determined.
Thus, the centrality measure $\psi'(\calI_R)$ for instance $\calI_R$ is unique, 
  for every nonempty $R\subset V$.

Now, by Axiom Spread Determination (Axiom~\ref{axiom:spread}), 
  $\psi'(\calI)$ is fully determined by the influence spread $\sigma_\calI$.
%Let $\sigma'_\calI(S) = \sigma_\calI(S) - |S|$ for every subset $S\subseteq V$.
By Lemmas \ref{lem:AI} and \ref{lem:oneone},
  $\sigma_\calI$ and $\sigma'_\calI$ have  one-to-one correspondence.
Thus, $\psi'(\calI)$ is fully determined by $\sigma'_\calI$.
Therefore, $\psi'$ can be viewed as a mapping from function
  $\sigma'_\calI$ to $\R^{|V|}$.
For each function $\sigma'_\calI$, we can view it as a vector of dimension 
$2^{|V|}-2$, which specifies for each $S\subset V$ with $S\not\in\{\emptyset,V\}$,
the value $\sigma'_\calI(S)$.
Note that $\sigma'_\calI(\emptyset) = \sigma'_\calI(V) = 0$, 
  so we do not need to specify the values for $S\in\{\emptyset,V\}$.

Next, we consider instance $\calI_R$ defined above with critical set $R$.
We show that all $\sigma'_{\calI_R}$ functions (treated as vectors)
with $R\not\in\{\emptyset,V\}$
are linearly independent in the space $\R^{2^{|V|}-2}$.
Suppose they are not linearly independent.
Then, for each such $R$, we have a number $\alpha_R \in \R$, such that
  $\sum_{R\not\in\{\emptyset,V\}} \alpha_R \sigma'_{\calI_R} = 0$, and
at least some $\alpha_R\ne 0$.
Let $S$ be the smallest set with $\alpha_S \ne 0$.
Consider any set $R$ with $|R| \ge |S|$ and $R\ne S$.
We have that $S \not\supseteq R$, 
and thus by the definition of critical set instance,  $P_\calI(S, S) = 1$.
This implies that $\sigma'_{\calI_R}(S) = \sigma_{\calI_R}(S) - |S| 
= |S| - |S| = 0$.
By the definition of $S$, we also know for any $R$ with $|R| < |S|$, $\alpha_R = 0$.
Therefore, we have:
 $$0 = \sum_{R\not\in\{\emptyset,V\}} \alpha_R \sigma'_{\calI_R}(S)
= \alpha_S \sigma'_{\calI_S}(S).$$
Finally, since $S \not\in \{\emptyset,V\}$ and $S$ is the critical set in $\calI_S$,
we have $\sigma'_{\calI_S}(S) = \sigma_{\calI_S}(S) - |S| = |V| - |S| > 0$.
Thus we obtain that $\alpha_S = 0$, a contradiction.
Therefore, vectors $\{\sigma'_{\calI_R}\}_{R\not\in \{\emptyset,V\}}$ are linearly independent.

Let the {\em null influence instance} $\calI^N$ to be the instance in which no seed set
has any influence except to itself, that is, For any $S\subseteq V$, 
$P_{\calI^N}(S,S) = 1$.
Since every node in $\calI^N$ is the same, by the Anonymity Axiom (Axiom~\ref{axiom:anonymity})
we have $\psi'_v(\calI^N) = 0$ for all $v\in V$.
That is, $\psi'_v(\calI^N)$ is uniquely determined.
In this instance, for any subset $S$, $\sigma'_{\calI^N}(S) = \sigma_{\calI^N}(S) - |S| = 0$.
Therefore, $\sigma'_{\calI^N}$ is the all-$0$ vector in $\R^{2^{|V|}-2}$.
This means that $\psi'(\vzero) = \vzero$.

With the above preparation, we can use the Bayesian Axiom (Axiom~\ref{axiom:bayesian})
	and Lemma~\ref{lem:linearmap} to argue that for any influence instance $\calI$, 
	if $\sigma'_\calI = \sum_{R\subseteq V, R\not\in \{\emptyset, V\}} \lambda_R \cdot 
			\sigma'_{\calI_R}$, then
		$\psi'(\sigma'_\calI) = \sum_{R\subseteq V, R\not\in \{\emptyset, V\}} \lambda_R \cdot 
			\psi'(\sigma'_{\calI_R})$, where we identify notation $\psi'(\sigma'_\calI)$
			with $\psi'(\calI)$.
Since we have argued above that  $\psi'(\calI_R)$ are uniquely determined for
	all $R \not\in \{\emptyset, V\}$, we know that $\psi'(\calI)$ is uniquely determined.
\end{proof}

\begin{theorem}
The Shapley centrality $\psi^{Shapley}$ is the unique centrality measure that satisfies
axiom set $\cA_\sigma$ (Axioms \ref{axiom:anonymity}, \ref{axiom:normalization},
	\ref{axiom:sink} -\ref{axiom:spread}).
\end{theorem}
\begin{proof}
This is directly implied by Lemmas~\ref{lem:shapleycen}, 
	\ref{lem:oneone}, and \ref{lem:unique2}, and the trivial fact that
	$\psi^{Shapley}$ satisfies Axiom~\ref{axiom:spread}.
\end{proof}


